VERISCORE: Evaluating the factuality of verifiable claims in long-form text generation

Existing metrics for evaluating the factuality of long-form text, such as FACTSCORE (Min et al., 2023) and SAFE (Wei et al., 2024), decompose an input text into "atomic claims" and verify each against a knowledge base like Wikipedia. These metrics are not suitable for most generation tasks because they assume that every claim is verifiable (i.e., can plausibly be proven true or false). We address this issue with VERISCORE, a metric for diverse long-form generation tasks that contain both verifiable and unverifiable content. VERISCORE can be effectively implemented with either closed or fine-tuned open-weight language models, and human evaluation confirms that VERISCORE's extracted claims are more sensible than those from competing methods across eight different long-form tasks. We use VERISCORE to evaluate generations from 16 different models across multiple long-form tasks and find that while GPT-4o is the best-performing model overall, open-weight models such as Mixtral-8x22 are closing the gap. We show that an LM's VERISCORE on one task (e.g., biography generation) does not necessarily correlate to its VERISCORE on a different task (e.g., long-form QA), highlighting the need for expanding factuality evaluation across tasks with varying fact density.

==> sections/claim_verification.tex <==
\section{Claim verification}\label{sec:claim.verification}

After ensuring a reliable extraction prompt and fine-tuned Mistral-7B-Instruct-v0.2 model for the claim extraction task, we now focus on the claim verification step. It has two components: evidence retrieval and binary classification. \sectionref{subsec:evidence_retrieval} introduces the evidence retrieval step.  \ys{ToDo}

\subsection{Evidence retrieval}\label{subsec:evidence_retrieval}

Similar to \citet{longfact}, we use Google search API provided by Serper\footnote{\url{https://serper.dev/}} to retrieve the up-to-date information that is related to a claim. Different from \citet{longfact} who use a LLM to generate five queries per claim and retrieve three search results per query, we use the extracted claims themselves as search queries. From each query, we retrieve at most ten search results. In the current work, we use the title, snippet, and the link information returned by the API and combine all search results into an evidence list. 

\subsection{Human performance on claim verification}\label{subsec:human_performance_on_verification}

The claim verification task requires complex reasoning, as defined in \tableref{tab:claim_veri_def}. We conduct a human study with three annotators to better understand the task: (1) whether the task is well defined and the annotators can reach certain agreement, (2) what types of data fall into the \inconclusive~categories, (3) why the annotators disagree, (4) whether it is needed to have 10 search results, and (5) what the distribution of the scenarios in \tableref{tab:claim_veri_def} is.
% The annotated data can be used to benchmark automatic verifiers.

\noindent \textbf{Data} We sampled 320 GPT4-extracted claims from  the eight domains from our newly generated model data in \appendixref{appendix:ft_claim_extraction}. Evidence is retrieved described in \sectionref{subsec:evidence_retrieval}. The 320 <claim, evidence list> pairs are split into 50 and 90 $\times$ 3 subsets. All annotators did the 50 split for agreement estimation and one of the 90 splits. 

\noindent \textbf{Task} For each item, the annotators were asked to make two types of decisions: (1) \textit{evidence level}: determine if each search result supports, contradicts, or provides insufficient information (inconclusive) about the claim; (2) \textit{claim level}: whether the claim is \supported, \contradicted, or being \inconclusive~w.r.t. the overall evidence.%\footnote{The task instruction and interface can be seen here: \url{https://docs.google.com/document/d/1xGl7gYZayCRpPRneJnb0Va1RnqZ4AbJhD9sv9SbLQUc/edit?usp=sharing}.}

\noindent \textbf{Human agreement} The agreement result shows that the claim verification task is well-defined and feasible. Out of the 50 triple-annotated items, 41 (82\%) had all three annotators in complete agreement. In 7 (14\%) other items, two annotators reached a consensus. The Fleiss $\kappa$ is $0.7316$ (substantial agreement \citealp{landis1977measurement}). 

Among the 41 fully agreed items, the annotators chose the \supported~label 26 times, and \inconclusive~15 times. There is no agreement on the \contradicted~label. Below, we closely look at the \inconclusive~cases and the rest 9 items that the annotators did not reach a full consensus. Concrete examples are in \appendixref{appendix:human_study_on_veri}. 

\noindent \textbf{Reasons of being inconclusive} Two reasons led the annotators to judge a claim as inconclusive w.r.t.\ its retrieved evidence. Examples are in \tableref{tab:ex_of_inconclu_cases}. First, a claim is too general to be verified (e.g., unclear referent). Second, there is no direct mentioning of a part of the claim or no evidence verifies the connection between the parts of a claim. There is no Inconclusive (b) cases (\tableref{tab:claim_veri_def}) among the 50 items. That means no item is marked as \inconclusive~because there are both supporting and contradicting search results. Beyond the triple-annotated data, only 7 items were marked as \inconclusive~because there are both supporting and contradicting search results.
% https://docs.google.com/document/d/1ggE5k0juYPS-YptqQW0CgCsDrFGF1oEgTpVnI_l7h74/edit

\noindent \textbf{Sources of disagreement} After inspecting the 9 items on which the annotators did not fully agree, we conclude 4 sources of disagreement. Examples are in \tableref{tab:ex_of_disagree_cases}. First, an annotator made a mistake (e.g., misread a name). Second, there is disagreement in the interpretation of the claim and evidence (e.g., \textit{can} in the claim vs.\ \textit{could} in the evidence or an ambiguous referent). Third, the claim is complex and long, hence, is hard to verify. Fifth, the evidence indirectly supports the claim which means intermediate reasoning process is needed. 

\noindent \textbf{Top search results are more informative.} We consider a search result as informative if it is marked as supporting or contradicting a claim. We analyzed the frequency with which search results were deemed informative. The first five search results show higher utility, with over 30\% being useful---the highest being the first search result at 35.56\%. For search results six to nine, their usefulness percentages range from 26.99\% to 29.16\%. The utility of the last search result drops to only 13.30\%.

\noindent \textbf{Only over half of the claims are \supported.} We analyzed the distribution of the claim level labels. For the triple-annotated data, we use the majority vote, if there is one, as the final label. Otherwise, the label is \inconclusive. Results in \tableref{tab:claim_veri_def_distribution} show that only 55\% of the claims are supported.

\begin{table}[h!]
\fontsize{6}{8}\selectfont
\centering
\resizebox{0.82\columnwidth}{!}{%
\begin{tabular}{@{}p{2cm}p{0.6cm}p{0.6cm}@{}}
\toprule
\textbf{Scenario}  & \textbf{Count} & \textbf{\%} \\ \midrule
Claim supported    & 176 & 55\%  \\
Claim contradicted & 9   & 2.8\% \\
Inconclusive (a)   & 128 & 40\%  \\
Inconclusive (b)   & 7   & 2.2\% \\\midrule
Total              & 320 & 100\% \\\bottomrule
\end{tabular}%
}
\caption{The distribution of the four scenarios (\tableref{tab:claim_veri_def}) that can happen in the claim verification step according to our human study in \sectionref{subsec:human_performance_on_verification}. 
}
\label{tab:claim_veri_def_distribution}
\end{table}

In order to understand whether the inconclusive cases can be verified/falsified by checking the full web page of the returned search results, we randomly picked 15 inconclusive cases and tried to manually verify them. It turns out that two claims are too underspecified to be verified (i.e., no clear referent). Only one claim can be verified by a copyright notice at the bottom of the full web page. For the other 12 cases, we used Google search to find more evidence but only one of them was weakly contradicted by a popular science article.\footnote{The claim is ``As a battery discharges, the chemical reactions inside the battery slow down.'' The article (\href{https://newsmartsafe.com/industry-news/battery-discharge}{link}) states ``When a battery is discharged, chemical reactions within the battery cells facilitate the movement of electrons from the negative terminal (anode) to the positive terminal (cathode) [...].'' If ``As a battery discharges'' is describing the status change of a battery from not discharging to discharging, the article implies that the chemical reactions become active but not slowing down. However, if the claim is understood as ``as a battery continues to discharge'', the article does not mention anything about chemical reactions slowing down gradually.} Others remain agnostic.

% https://docs.google.com/spreadsheets/d/1tmdrQZRZCQawGS3dU-ORKQUpHid6SdNwq1L1JI_HnLE/edit?usp=sharing

\subsection{Fine-tune open-source models for claim verification}\label{subsec:ft_for_claim_verification}

Similar to the claim extraction task, we fine-tune Llama3-8B-Instruct and Mistral-7B-Instruct-v0.2 for an open-source claim verifier. We report the details in \appendixref{appendix:ft_claim_verification}. When choosing the best checkpoint, we emphasize the model performance on both the \supported~and \unsupported~claims to avoid bias towards one label. By doing so, we aim to create a verifier that is equally adept at identifying valid claims as well as recognizing unsupported claims, thus enhancing the reliability and robustness of the verification process. We open-source the best checkpoint from Llama3-8B-Instruct and use it for further experients.

==> sections/data_and_llm.tex <==
\section{Data domains and studied LLMs}\label{sec:data_and_llm}
\ys{merge into sec 6}
As a factuality evaluation pipeline, \name\ aims to operate on a wide range of domains. It is developed, tested, and benchmarked using the eight domains of model outputs. The datasets include prompts requiring highly fact-dense responses (e.g., long-form question answering such as AskHistorians and ELI5), moderately factual responses (e.g., ShareGPT), and fictional responses (e.g., WritingPrompts). We also collected a dataset New Books that consists of 10 paragraphs from each of 20 non-fictional books that are published between 2023 and 2024. Models are required to generate a continuation of the paragraphs. Details of each domain can be found in \tableref{tab:eight_datasets_for_ft} and \tableref{tab:new_book_dataset}.

% \input{emnlp2023-latex/tables/fine-tune_model_datasets}

We evaluate the factuality capabilities of 16 close- and open-source language models of different sizes or versions. The three largest model families are the GPT, Claude3, and Mistral/Mixtral models. We also evaluate language models of various sizes, for example, Qwen1.5-1.8B-Chat, Gemma-2B-it, OLMo-7B-Instruct, Vicuna-7B-v1.5, and DBRX Instruct (132B). Details of the models are in \tableref{tab:simple_12_models_for_response_gen}. To generate model responses for evaluation, the models are prompted with their default hyperparameters and a maximum token length set to 1024. The prompts are sampled from the datasets in \tableref{tab:eight_datasets_for_ft}. We use the original prompts but prepend the instruction ``Write a story based on the following writing prompt'' to the prompts in WritingPrompts, and, for New Books, ``Generate a continuation of the following text. The continuation should be objective and factual''.

% \input{emnlp2023-latex/tables/simple_models_for_response_gen}

% \subsection{Comparison to \factscore~and SAFE}

% \input{emnlp2023-latex/tables/ours_safe_factscore_comparison}

% \tableref{tab:our_factscore_safe}

==> sections/fine_tune_models.tex <==
\section{Fine-tune open-source models for claim extraction and verification}\label{subsec:ft_for_claim_extraction}

% To facilitate the factuality evaluation of different text domains, we fine-tune Llama3-8B-Instruct and Mistral-7B-Instruct-v0.2 (henceforth Llama3 and Mistral) to create a deterministic and cost-efficient claim extractor and verifier with performance comparable to the best LLMs. We detail the fine-tuning process of each task below.

\subsection{Fine-tuned claim extractor}

We fine-tune Llama3 and Mistral on GPT4-extracted claims to obtain a claim extraction model returns deterministic claim extraction outputs. We compared the outputs from our best fine-tuned model Mistral to GPT4 on 300 data points. The results show that 46\% of our model's outputs exactly match the ones from GPT4. About 20\% of the outputs from the both models are almost equivalent. Among the rest of the outputs, our model performs comparably to GPT4 (Rouge2 = 0.758, RougeL = 0.801). Details of the fine-tuning process and the quality analysis are in \appendixref{appendix:ft_claim_extraction}.

\subsection{Fine-tuned claim verifier}\label{subsec:ft_for_claim_verification}

We fine-tune Llama3 and Mistral for an open-source claim verifier. Training data are generated from GPT-4o. Details of the fine-tuning are reported in \appendixref{appendix:ft_claim_verification}. We aim for a verifier that is equally adept at identifying valid claims as well as recognizing unsupported ones. Hence, when choosing the best checkpoint, we emphasize the model performance on both the \supported~and \unsupported~claims to avoid bias towards one label. Llama3 returns the best performance. We open-source its best checkpoint and use it for further experiments.

==> sections/issues.tex <==
\section{Issues in decompositional factual evaluation}\label{sec:quality_analysis}

% We built on previous work and proposed \name, a pipeline of evaluating models' factuality ability. It performs significantly better than \factscore~and SAFE in claim extraction and comparably to the best large language model and human performance on claim verification. However, 

This section examines \name's performance across different domains and show that the decompositional factual evaluation is not always practical and has its limitation. Three issues are identified: (1) it is hard to decompose model responses into short claims, (2) search snippets are not enough for verification, and (3) precision and $F_1@K$ are vulnerable metrics. Examples are provided in \tableref{tab:false_irrelevant}.

\input{tables/issues}

\subsection{Not all claims can be decomposed and short}

Decomposing model responses before checking factuality helps locate factual errors. Shorter, self-contained claims are desired because they are easier to be verified. However, claims extracted from domains other than LongFacts \citep{longfact} and \factscore~\citep{factscore} are often longer. 

To confirm this, we randomly sampled 200 claims from \citet{factscore}'s model extracted claims and 200 claims extracted by GPT4 from GPT4-0125 generated ELI5 responses. On average, \factscore's claims have 7 words, with the longest claim having 18 words. In contrast, our claims extracted from ELI5 on average have 12 words, with the longest being 25 words. We manually analyzed 166 ELI5 claims that are longer than 7 words. Only 16\% of them can be further decomposed. This is merely because they contain \textit{and} or \textit{or}. As an example, after decomposing, the length of the first claim in \tableref{tab:false_irrelevant} is not significantly shorter because the core content of the claims cannot be decomposed.
% Decompositing it will also result in 4 claims: \{traverls, crusaders\} $\times$ \{clean, consistent\}.

Occasionally, shorter claims can be extracted from a longer one. However, verifying the shorter claims does not entail verifying the longer one, for example, the second claim in \tableref{tab:false_irrelevant}. The content before and after \textit{solidified} can be verified independently. However, to verify \textit{solidified}, the whole claim cannot be decomposed.

% \subsection{Length affects \name}

% Longer claims present challenges for verification. A point biserial correlation test on the human-annotated claims in \sectionref{subsec:human_performance_on_verification} reveals a moderate positive correlation between claim length and their labels ($r_{pb} = 0.283, p<0.001$).\footnote{Due to the limited number of the \contradicted~claims, we combined the \contradicted~and \inconclusive~claims into one label.} 

% yixiao/atomic_claims/code/2ndHumanEval_claim_search_res_verify/result_analysis/corr_len_label_my_biserialr.py

\subsection{Search snippets are not enough for verification}\label{subsec:snippets_not_enough}

Same as SAFE, \name\ utilizes Google Search snippets to access the latest world knowledge for verifying claims. However, our analysis of the inconclusive cases in \sectionref{subsec:human_performance_on_verification} reveals that the snippets are insufficient. One reason is that some claims require detailed reasoning to verify the connections among their components (see the second claim in \tableref{tab:false_irrelevant}). Snippets do not offer enough background for such reasoning. Additionally, models may generate sentences that appear plausible but do not hold up under scrutiny, for example the third claim in \tableref{tab:false_irrelevant}). Addressing such claims requires expertise in a particular field or might even be impractical when the claims involve non-existent facts. 

With the current system, when a claim is judged as \unsupported~without direct contradicting evidence, it is impossible to decide whether a model hallucinates because it is beyond what reasoning over search snippets can achieve. The presence of seemingly plausible claims indicates the need to move beyond string or semantic matching for verifying model-generated content as they fail to uncover possible hallucination.

\subsection{Precision and $F_1@K$ are vulnerable}

\ys{length sensitive, relevance check}

\factscore~uses factual precision as the metric for factual evaluation but fails to penalize models that do not generate sufficient factual content. SAFE addresses this by proposing $F_1@K$, a metric that considers precision and recall. It requires a model to generate at least $K$ supported fact to achieve perfect recall, penalizing models that generate less factual content, such as gpt-3.5-turbo-1106 (see \figureref{fig:model_resp_heatmap} and fn. \ref{fn:gpt_len}).

Despite the improvement made by $F_1@K$, the metric does not penalize abstained models and can be exploited by having $K$ factual but irrelevant claims. SAFE attempts to mitigate this by removing irrelevant claims before verification but the relevance check is not reliable, as discussed in \sectionref{subsec:issue_in_safe}. As another example, SAFE's relevance check judges the last claim in \tableref{tab:false_irrelevant} as irrelevant, even though the sentence is crucial to answering the question by referencing an existing castle. 


==> tables/claim_extraction_datasets.tex <==
\begin{table*}[]
\fontsize{8}{10}\selectfont
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lp{10cm}p{3cm}@{}}
\toprule
\textbf{Name}    & \textbf{Description}   & \textbf{Source}                                              \\ \midrule
Scruples       & Community judgements on real-life anecdotes from \href{https://reddit.com/r/AmItheAsshole}{r/AmItheAsshole} from November 2018 to April 2019           & \citet{lourie2021scruples}         \\[1mm]
CommonCrawl    & A corpus of raw web page data, metadata extracts, and text extracts & \href{https://commoncrawl.org/overview}{CommonCrawl} \\[1mm]
wikitext-103   & Wikipedia articles & \citet{merity2016pointer}          \\[1mm]
WritingPrompts & Story premises and stories written by online users on \href{https://reddit.com/r/WritingPrompts/}{r/WritingPrompts} & \citet{fan-etal-2018-hierarchical} \\[1mm]
ShareGPT       & User-shared conversations (prompts and responses) with ChatGPT on \url{ShareGPT.com} &    \citet{chiang2023vicuna}\textsuperscript{*}     \\[1mm]
ELI5           & Questions and layperson-friendly answers posted on \href{https://www.reddit.com/r/explainlikeimfive/}{r/explainlikeimfive} & Scraped by \citet{xu-etal-2023-critical}      \\[1mm]
AskHistorians   &  Questions and answers on history topics posted on \href{https://www.reddit.com/r/AskHistorians/}{r/AskHistorians}   & Same as above \\[1mm]

\factscore      & Biography text generated by PerplexityAI, InstructGPT, and ChatGPT & \citet{factscore}\\\bottomrule
\end{tabular}%
}
\caption{Datasets that are used in the human pair-wise evaluation in \sectionref{subsec:1stHumanEval} of our one-step extraction method and SAFE's two-step extraction pipeline. The first four datasets are non-QA data and the last three are QA-data. \\
\small{\textsuperscript{*}Data is downloaded from \href{https://huggingface.co/datasets/anon8231489123/ShareGPT_Vicuna_unfiltered}{anon8231489123/ShareGPT\_Vicuna\_unfiltered} on Hugging Face.}}
\label{tab:seven_datasets_for_claim_extraction}
\end{table*}



==> tables/fine-tune_model_datasets.tex <==
\begin{table*}[h!]
\fontsize{8}{10}\selectfont
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lp{10cm}p{3cm}@{}}
\toprule
\textbf{Name}  & \textbf{Description}  & \textbf{Source}  \\ \midrule
LongFact      & A prompt set of 38 topics generated by GPT-4; each topic has 2 types of prompts---object \& concept; we randomly sampled 10 prompts from 10 topics, with half of them being object and the other half being concept & \citet{longfact} \\[2mm]
FreshQA        & A dynamic QA benchmark whose answers can change w.r.t. updated world knowledge; we randomly sampled 200 questions with a true premise from the never- and fast-changing categories in the test set of the April 1\textsuperscript{st} version  & \citet{vu2023freshllms} \\[2mm]
FreshBooks      & We collected 20 non-fictional books that are published in 2023 and 2024. Ten paragraphs are taken from each book. LLMs are prompted to generate a continuation given a paragraph & Current paper;\newline Details in \tableref{tab:new_book_dataset} \\[1mm]
% Others         & WritingPrompts \quad ShareGPT \quad ELI5 \quad AskHistorians \quad \factscore & See \tableref{tab:seven_datasets_for_claim_extraction} \\[1mm] 
WritingPrompts & Story premises and stories written by online users on \href{https://reddit.com/r/WritingPrompts/}{r/WritingPrompts} & \citet{fan-etal-2018-hierarchical} \\[1mm]
ShareGPT       & User-shared conversations (prompts and responses) with ChatGPT on \url{ShareGPT.com} &    \citet{chiang2023vicuna}\textsuperscript{*}     \\[1mm]
ELI5           & Questions and layperson-friendly answers posted on \href{https://www.reddit.com/r/explainlikeimfive/}{r/explainlikeimfive}  & Scraped by \citet{xu-etal-2023-critical}      \\[1mm]
AskHistorians   &  Questions and answers on history topics posted on \href{https://www.reddit.com/r/AskHistorians/}{r/AskHistorians}   & Same as above \\[1mm]

\factscore      & Biography text generated by PerplexityAI, InstructGPT, and ChatGPT & \citet{factscore}\\\bottomrule
\end{tabular}%
}
\caption{Datasets that are used for developing, test, and benchmark \name. \ys{merge table 6 and 12 and add a column "Human Eval" and "Dev". In the caption, explain what "Dev" is. Add in claim/sent ratio as a column?}}
\label{tab:eight_datasets_for_ft}
\end{table*}

==> tables/issues.tex <==
\begin{table*}[h]
\fontsize{9}{11}\selectfont
% \small
\centering 
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}p{16cm}@{}}
\toprule

\multicolumn{1}{c}{\textbf{\scalebox{1.1}{Search snippets are not enough for verification}}}\\\midrule

\textbf{Claim}: Japanese people encountered tigers in the form of stuffed animals before the Meiji era.

\textbf{Original model response}: ... Before the Meiji era (1868-1912), Japanese people would encounter tigers mainly through artwork, literature, and other forms of media. They would also see tigers in zoos and circuses, as well as in the form of stuffed animals and other souvenirs. ...

\textbf{Authors' note}: The claim is faithfully extracted from the original model response. It cannot be verified for two reasons. First, no search results online directly mention ``stuffed tiger'' and the time period before the Meiji era together. Second, the claim is vague in the sense of what ``Japanese people'' means. One search result states that ``The Japanese came across tigers on their forays into Korea in the late 16th century.'' However, it is unclear whether the Japanese who conducted these forays represent ``Japanese people''. Details and one more example are in \tableref{tab:seemingly_plausible}.\\\bottomrule

% \multicolumn{1}{c}{\textbf{\scalebox{1.1}{Precision and $F_1@K$ are vulnerable and SAFE's relevance check does not help}}}
% \\\bottomrule

% \textbf{Question}: At their peak, what did the insides of the most beautifully decorated castles look like? Today, castles seem to just be giant fortresses but I would like to know how they looked when they were fully furnished. How were they decorated? What treasures were stored there? Are there a few castles that were especially beautiful?

% \textbf{Human response}: It is quite a broad subject because castles varied quite a lot depending on location, time of construction and wealth of the constructor; u/valkine talked about Caenarfon Castle \href{https://www.reddit.com/r/AskHistorians/comments/26vvmz/were_castles_in_medieval_england_typically/}{(link)} specifically in another question \href{https://www.fortementein.com/wp-content/uploads/2021/03/p-le9102-1280x720.jpg}{(link)} is a part of the inside of \colorbox{yellow}{Castello Maniance in Siracusa, Italy. It was built from 1232 to 1239} during a large castle-construction effort by Emperor Frederick II.  I do find it particularly beautiful but this doesn't really say much about what other castles looked like

% \textbf{Extracted claim}: Castello Maniance in Siracusa, Italy was built from 1232 to 1239.

% \textbf{Authors' note}: A reliable factuality metric should check whether the generated factual content is relevant to the prompt. SAFE's relevance check aims at this but identifies crucial content as irrelevant.\\\midrule

\end{tabular}%
}
\caption{Examples illustrating challenges in claim extraction and verification, the limitations of search snippets for fact-checking, and relevance assessment.}
\label{tab:false_irrelevant}
\end{table*}

==> tables/models_for_response_gen.tex <==
\begin{table*}[h!]
\fontsize{8}{10}\selectfont
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}cp{4.5cm}p{2cm}p{1cm}p{1.5cm}p{3cm}@{}}
\toprule
\textbf{API}   & \textbf{Name}   & \textbf{\# of Parameters}  & \textbf{Open}  & \textbf{Release} & \textbf{Reference} \\ \midrule
\multirow{4}{*}{\rotatebox{90}{\fontsize{7}{8}\selectfont \hspace{5pt}OpenAI}} & gpt-4-0125-preview & --- & \xmark & 2024-01-25 & \multirow{3}{*}{\citet{DBLP:journals/corr/abs-2303-08774}} \\
                        & gpt-3.5-turbo-1106 & --- & \xmark & 2023-11-06 &  \\
                        & gpt-3.5-turbo-0613 &  --- & \xmark & 2023-06-13 &  \\\midrule
\multirow{3}{*}{\rotatebox{90}{\fontsize{7}{8}\selectfont Anthropic}} & claude-3-haiku-20240307 & --- & \xmark & 2024-03-04 & \multirow{3}{*}{\citet{Anthropic2023Claude}} \\
                           & claude-3-sonnet-20240229& --- & \xmark & 2024-03-04 & \\
                           & claude-3-opus-20240229  & --- & \xmark & 2024-03-04 & \\\midrule
\multirow{6}{*}{\rotatebox{90}{\fontsize{7}{8}\selectfont TogetherAI\hspace{10pt}}}& mistralai/Mistral-7B-Instruct-v0.1     & 7.3B & \cmark & 2023-09-27 & \multirow{4}{*}{\citet{Jiang2023Mistral7, Jiang2024MixtralOE}} \\
                           & mistralai/Mistral-7B-Instruct-v0.2    & 7.3B & \cmark & 2023-09-27 & \\
                           & mistralai/Mixtral-8x7B-Instruct-v0.1  & 46.7B (12.9B) & \cmark & 2023-12-11 & \\
                           & mistralai/Mixtral-8x22B-Instruct-v0.1 & 141B (39B)  & \cmark & 2023-12-11 & \\\cmidrule(l){2-6}
                           & allenai/OLMo-7B-Instruct & 7B & \cmark & 2024-02-01 & \citet{groeneveld2024olmo} \\\cmidrule(l){2-6}
                           & databricks/dbrx-instruct & 132B (36B) & \cmark & 2024-03-27 & \citet{DBRXblog} \\ \bottomrule
\end{tabular}%
}
\caption{Description of models used to generate responses from training data. The parameter count indicates the total number of active parameters. \ys{@yekyung: can you explain the meaning of numbers in brakcets?} Dashes mean that the model providers do not officially disclose the number of parameters.}
\label{tab:12_models_for_response_gen}
\end{table*}

==> tables/ours_safe_factscore_comparison.tex <==
\begin{table*}[h!]
\fontsize{8}{10}\selectfont
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}p{1.885cm}p{3cm}p{3cm}p{3cm}@{}}
\toprule
\textbf{Evaluatior}   & \textbf{Evaluated topic} & \textbf{Claim extraction} & \textbf{Claim verification}\\ \midrule

\factscore\newline\citep{factscore} & Biography only & Sentence by sentence w/o resolving vague references & One Wikipedia article,\newline ChatGPT as verifier\\\midrule

SAFE\newline \citep{longfact} & 38 fact-seeking topics, most questions are \textit{who is}, \textit{what is}, and \textit{can you tell me about} & Three-step extraction:\newline - \factscore's prompt\newline - Vague reference Revision\newline - Irrelevant claim removal & Google search results,\newline LLMs as verifier \\\midrule

Ours & \textbf{Topics w/ varying degrees of factuality} (e.g., ELI5, ShareGPT, and WritingPrompts). & A fine-tuned model that resolves vague referents and \textbf{matchs GPT4's performance} & Google search,\newline \textbf{Fine-tuned verifier} \\\bottomrule

\end{tabular}%
}
\caption{An overview of our evaluator compared to \factscore~\citep{factscore} and SAFE \citep{longfact}. While \factscore~and SAFE focus solely on fact-dense text, we investigate factuality evaluation in topics with different degrees of fact density. We also provide fine-tuned models for the claim extraction and verification that achieve comparable performance to GPT4 and GPT-4o.
}
\label{tab:our_factscore_safe}
\end{table*}

==> tables/seemingly_plausible_claims.tex <==
\begin{table*}[h]
\fontsize{10}{12}\selectfont
% \small
\centering 
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}p{16cm}@{}}
\toprule
\multicolumn{1}{c}{\textbf{\scalebox{1.1}{Example 1}}}
\\\midrule

\textbf{Claim}: Linguistic Citizenship views language use as a way of enacting disaffiliation with imagined communities.\newline

\textbf{Query 1}: What is linguistic citizenship\newline
\textbf{Result}: Linguistic Citizenship is an attempt to work through a blueprint for language for navigating living the complexities of a diverse and difficult world in conviviality (and convivial contest) with different Others.\newline

\textbf{Query 2}: What are imagined communities\newline
\textbf{Result}: Imagined communities refer to groups of people, not immediately tangible and accessible, with whom we connect through the power of the imagination. In our daily lives we interact with many communities whose existence can be felt concretely and directly … however, these are not the only communities with which we are affiliated … in imagining ourselves bonded with our fellow compatriots across space and time, we can feel a sense of community with people we have not met, but perhaps hope to meet one day.\newline

\textbf{Authors' note}: The search results using the claim itself as the query from Google Search do not mention \textit{linguistic citizenship} and \textit{imagined community} together. During the manual verification, beyond what Google Search already returned, we searched about \textit{linguistic citizenship} and \textit{imagined community}. The results are below. \newline
Based on the results, we sense that if one wants to disaffiliate with their imagined communities, they can simply stop imagining themselves bonded with such communities. ``Imagined community'' and ``use language as a way of enacting disaffiliation'' do not logically form a coherent connection.\newline \midrule

\multicolumn{1}{c}{\textbf{\scalebox{1.1}{Example 2}}}
\\\midrule

\textbf{Claim}: Japanese people encountered tigers in the form of stuffed animals before the Meiji era.\newline


\textbf{Original model response}: Before the Meiji era (1868-1912), Japanese people would encounter tigers mainly through artwork, literature, and other forms of media. They would also see tigers in zoos and circuses, as well as in the form of stuffed animals and other souvenirs.\newline

\textbf{Search result 1}\newline
Title: I've seen Japanese artwork from the Edo era and before depicting ...\newline
Content: ... Japanese person encounter a tiger before the Meiji era? ... Even baby tigers was captured and be made as stuffed. ... Are tigers semiaquatic animals ...\newline
Link: https://www.quora.com/I-ve-seen-Japanese-artwork-from-the-Edo-era-and-before-depicting-tigers-Did-tigers-ever-inhabit-the-islands-of-Japan-If-not-how-might-a-Japanese-person-encounter-a-tiger-before-the-Meiji-era\newline

\textbf{Search result 2}\newline
Title: I've seen Japanese artwork from the Edo era and before depicting ...\newline
Content: I've seen Japanese artwork from the Edo era and before depicting Tigers. Did tigers ever inhabit the islands of Japan?\newline
Link: https://www.reddit.com/r/AskHistorians/comments/p47bj6/ive\_seen\_japanese\_artwork\_from\_the\_edo\_era\_and/ \newline

\textbf{Authors' note}: We confirmed that the claim is faithfully extracted from the original model response (see below). The claim cannot be verified for two reasons. First, no search results (returned by different queries) directly mention ``stuffed tiger'' and ``Meiji era'' together. Only one search result mentions ``stuffed''. However, the \href{https://www.quora.com/Why-are-there-so-few-Siberian-tigers/answer/Dong-Yoon-Lee}{web page} does not mention the Meiji era. The second reason is that the claim is vague in the sense of what ``Japanese people'' means. The web page of search result 2 states that ``The Japanese came across tigers on their forays into Korea in the late 16th century.'' However, it is questionable whether the Japanese who conducted these forays represent ``Japanese people''. Given these reasons, we were not able to verify or falsify the claim.\newline
\bottomrule

\end{tabular}%
}
\caption{Examples of seemingly plausible but hard to be verified/falsified claims.}
\label{tab:seemingly_plausible}
\end{table*}
